Radial multipliers on mixed-norm spaces over free groups

The problem of Fourier summation on free groups remains open and challenging. More precisely, if $B_N(e)$ are the balls of radius $N$ on $\mathbb{F}_r$, it is still open whether they induce a uniformly bounded family of Fourier multipliers on the non-commutative $L_p$-spaces associated with their regular von Neumann algebras. Nevertheless, progress has been made. In particular, Kuhn and later Bozejko/Fendler showed that the ball multipliers are non-uniformly bounded when restricted to the radial subalgebra of the free group if $p \not\in (\tfrac{3}{2}, 3)$. We will produce a converge to their results by introducing mixed $L_p(L_2)$-norms given by \[ \| x \|_{p, \mathrm{mix}} := \big\| \mathbb{E}_{\mathrm{rad}} \big[ x^\ast \, x \big]^\frac12 \big\|_p, \] where $\mathbb{E}_\mathrm{rad}$ is the expectation onto the radial subalgebra. These spaces can be seen as free analogues of the mixed $L_p$-radial/$L_2$-angular norms studied in the Euclidean case by Mockenhaupt, Rubio de Francia and A. Cordoba. We show that the ball multipliers are uniformly bounded on these mixed-norm spaces exactly when $p \in (\tfrac{3}{2}, 3)$, thus confirming intuitions going back to Biane about the dual of the free group behaving as a $3$ dimensional object. Lastly, using Fourier-Schur comparison, we show that the balls associated with the $q$-convex deformations of the word length function of $\mathbb{F}_r$ have divergent completely bounded norms as multipliers on $L_p$ spaces if $q > 1$. When $q = 1$, recent results on radial Schur multipliers show that the strategy cannot possibly work.

==> blank.tex <==
As a key tool, we employ the following \emph{Plancherel theory} of free groups \cite{FP1983}. Let $\partial\Fr$ be the Poisson boundary of the free group $\Fr$ and $\lambda$ be the left regular representation of $\Fr$, see Section~\ref{Preliminaries}. Then, up to unitary equivalence, the representation $\lambda$ can be decomposed into a direct integral of irreducible representations $(\pi_s)_{s\in I}$ of $\Fr$ on $L^2(\partial\Fr)$. In particular, the group von Neumann algebra $\mathcal{L}\Fr$ can be embedded into the algebra of operator-valued functions $L^\infty(I)\,\bar{\otimes}\, B(L^2(\partial\Fr))$, and we may explicitly write down a unitary transformation
\[
\Phi\colon L_2(\mathcal{L}\Fr)\to L_2(I,dm_r;L_2(\partial\Fr)).
\]
Our arguments are based on the following observations and ideas.
\begin{enumerate}
	\item The Plancherel theory above provides an appropriate framework for a free analogue of radial-angular analysis on the von Neumann algebra $\mathcal{L}(\Fr)$. As a rough geometric intuition, for an element $\gamma \in \Fr$, if we write $\lambda(\gamma) \in \mathcal{L}(\Fr)$ as an element in $L^\infty(I)\,\bar{\otimes}\, B(L^2(\partial\Fr))$ and keep in mind the standard identification $L_\infty(I) \cong \mathcal{L}\Fr^{\mathrm{rad}}$, the component on $I$ captures how $\lambda(\gamma)$ acts between the radial spheres in the Cayley graph of $\Fr$, while the component on $\partial\Fr$ captures how $\lambda(\gamma)$ shifts the vertex directions on the graph.
	\item Any radial Fourier multiplier map $T_\varphi\colon \lambda(\gamma)\mapsto \varphi(\gamma)\lambda(\gamma)$ for a radial function $\varphi\colon\Fr\to\mathbb{C}$ can be interpreted as a diagonal-block operator-valued integral operator in an explicit way. More precisely, we may find a decomposition $L_2(\partial\Fr)=\bigoplus_{m\geq 0}\cH_m$ into Hilbert subspaces $\cH_i$, and a complete orthogonal system $\{Q_{m,n}\}_{n\ge m}$ of $L_2(I)$, such that for all bounded radial functions $\varphi\colon\Fr\to\mathbb{C}$, the conjugated Fourier multiplier map $\widetilde T_\varphi\coloneqq \Phi\circ T_\varphi\circ\Phi^{-1}$ on $L_2(I)\otimes L_2(\partial\Fr)$ satisfies, for all $i\geq 0$:


This key ingredient helps reduce the study of noncommutative Fourier multipliers to that of spectral multipliers $(R_{\varphi,i})_i$ on classical Hilbert-space-valued function spaces, which is much more manageable. This new interpretation is one of the core technical analyses in this paper, and relies essentially on the geometry of Cayley graphs and the analysis of irreducible representations of the free group on its Poisson boundary.
In the case of ball multipliers with $\varphi =\chi_{\{|\cdot |\leq N\}}$, we may carry out a delicate analysis of the spectral multipliers $(R_{\varphi,i})_i$. Indeed, the aforementioned orthogonal system $(Q_{n,i})_n$ can be explicitly computed as a deformation of Chebyshev polynomials. A careful analysis of such orthogonal systems yields, in Section~\ref{subsec: generalization of Pollard's arguments}, a decomposition
$$R_{\varphi,i} = \text{a \emph{weighted Hilbert transform} + a regular integral operator}.$$
This allows us to perform the desired weighted $L_2$ analysis of $R_{\varphi,i}$ using singular integral theory with $A_p$ weights. 




We will also use the following stability of the Schur multiplier $S_p$-boundedness under measurable changes of variables. Let $\psi: (\Omega_1, \mu_1) \to (\Omega_2, \mu_2)$ be a measurable transformation and $M \circ (\psi \otimes \psi) (\omega, \eta) = M(\psi(\omega), \psi(\eta))$, then
\begin{equation}
    \label{eq: change of variable}
    \big\| S_{M \circ (\phi \otimes \phi)}: S_p(\Omega_1) \to S_p(\Omega_1) \big\| 
    \leq \big\| S_{M}: S_p(\Omega_2) \to S_p(\Omega_2) \big\|,
\end{equation}
and the same follows for complete norms; see \cite{Parcet2024Idempotentschur}.




Let \(F: \{1/2+\mathrm it:\ t\in [0,\pi/\log(2r-1)]\} \to I\) be a bijection defined by
\begin{equation}\label{F-def}
    F(z) = \frac{1}{2r}\big((2r-1)^z + (2r-1)^{1-z}\big),
\end{equation}
and let \(\pi_s\) be the action of \(\Fr\) on \(L_2(\partial\Fr)\) given by
\begin{equation}\label{pi-def}
	\pi_s(\gamma)\xi(\cdot) := P(\gamma,\cdot)^{F^{-1}(s)}\,\xi(\gamma^{-1}\cdot),
	\qquad s\in I,\ \gamma\in\Fr,\ \xi\in L_2(\partial\Fr).
\end{equation}
It is straightforward to verify that $\pi_s$ defines a unitary representation of $ \mathbb F _r$ on $L_2(\partial\Fr)$. This parametrized family of representations $(\pi_s ) _{s\in I}$ constitutes the \emph{principal series} of \(\Fr\), the analogue of the principal series for semisimple Lie groups.

\iffalse 
{\color{red}
Let $\varphi:\Fr \to \mathbb C$ be a radial function. To obtain the kernel for \(T_a\), we introduce the following \(T_a\)-invariant subspaces. For integers \(m\ge 0\) and \(n\ge m\), define
\[
V_{m,n}
\coloneqq
\operatorname{span}
\left\{ 
\cD_m(\lambda(\gamma )): |\gamma |=n,\gamma\in\mathbb F_r
\right\},
\]
which means \(V_{m,n}\) is the subspace of \(\cL \Fr\) consisting of the \(m\)-th difference components associated with Fourier coefficients supported on the sphere of radius. Then,
\[L^2(\mathcal{L}(\mathbb F_r)) = \bigoplus_{m=0}^\infty \bigoplus_{n= m}^\infty V_{m,n} .\]
More explicitly, by \eqref{defEm},
\[
V_{m,n}
=
\operatorname{span}
\Big\{
\frac{c(m)}{c(n)}\lambda(\chi_{S(\gamma^{(m)},n)})
-
\frac{c(m-1)}{c(n)}\lambda(\chi_{S(\gamma^{(m-1)},n)})
:
|\gamma |=n
\Big\},\quad m\ge 1,\ n\ge m.
\]
In the case \(m=0\), the space \(V_{0,n}\) is the radial component on the sphere of radius \(n\), namely
\(
V_{0,n}
=
\operatorname{span}
\left\{
\lambda(\mu_n)
\right\}.
\)
Let \(P_{m,n}\) denote the orthogonal projection from
\(L_2(\cL \Fr)\) onto \(V_{m,n}\). Since the Fourier support of each element of \(V_{m,n}\) is contained in the sphere of radius \(n\),
the subspace \(V_{m,n}\) is invariant under \(T_a\). 
Therefore, for every \(x\in \cL \Fr\), using the decomposition associated with the projections \(P_{m,n}\), we obtain
\begin{equation}\label{Tvarphi_Pmn}
	\begin{aligned}
		T_a(x)
		&=
		\sum_{m\ge 0}\sum_{n\ge m}
		T_a\bigl(P_{m,n}(x)\bigr) \\
		&=
		\sum_{m\ge 0}\sum_{n\ge m}
		\varphi(n)
		P_{m,n}(x).
	\end{aligned}
\end{equation}
}
\fi

==> previous_versions/introduction_free_ball_mult1.tex <==

Let \(G\) be a discrete group with left regular representation \(\lambda:G\to B(\ell_2(G))\) given by \(\lambda(\gamma)\delta_\eta=\delta_{\gamma \eta}\), where \(\delta_\gamma\)'s form the unit vector basis of \(\ell_2(G)\). Let \(\mathcal L(G)\) denote the group von Neumann algebra of \(G\), namely the weak operator closure of the linear span of \(\lambda(G)\). We consider the standard normalized trace  \(\tau(x)=\langle x\delta_e,\delta_e\rangle\), where \(e\) denotes the identity of \(G\). 
For \(1\le p<\infty\), let \(L_p(\mathcal L(G),\tau)\) denote the associated noncommutative \(L_p\)-space (see \cite{PX2003}), endowed with the norm
$$\|x\|_{L_p(\mathcal{M})}= \tau(|x|^p)^{1/p},\; x\in \mathcal{M},$$
where $|x|=(x^*x)^{\frac{1}{2}}$ is the modulus of $x$.
Each \(x\in L_1(\mathcal L(G))\) admits a Fourier expansion
\[x\sim\sum_{\gamma\in G}\widehat{x}(\gamma)\lambda(\gamma)\]
with \(\widehat{x}(\gamma)=\tau(x\lambda(\gamma)^*)\) so that \(\tau(x)=\widehat{x}(e)\). Given a function \(\varphi: G \to\mathbb C\), the associated Fourier multiplier is defined by
\[
T_\varphi : \sum_\gamma \widehat{x}(\gamma)\lambda(\gamma) \mapsto \sum_\gamma \varphi(\gamma) \widehat{x}(\gamma)\lambda(\gamma).
\]

The origins of noncommutative Fourier multiplier theory can be traced back to Haagerup’s pioneering work on free groups \cite{Haa1978}. By employing Fourier multiplier methods, Haagerup constructed radial multiplier approximations on free groups, 
thereby solving the longstanding problem of Grothendieck’s approximation property for the reduced $C^*$-algebras of free groups.
Later, Haagerup, together with de Canni\`ere and Cowling \cite{DH1985,CH1989}, studied completely bounded Fourier multipliers on the Fourier algebras of simple Lie groups. This work led to
fundamental notions such as the Haagerup property, rapid decay, and weak
amenability. Moreover, these tools have played a crucial role in the work of Popa, Ozawa, and Vaes \cite{OP2010,PV2014}, with significant applications to deformation/rigidity theory, strong solidity, and related areas.




% all of which can be viewed as boundedness or approximation
%properties of suitable noncommutative Fourier--Schur multipliers. In this
%way, the estimates of Fourier multiplier  were shown to be not merely analytic tools, but also  a
%source of invariants for groups,
%group $C^*$-algebras, and group von Neumann algebras.

Fourier multiplier plays an important role in classical analysis, and one of the the basic problem is to determine the \({L_p}\)-boundedness of the multiplier. The works mentioned above may be regarded as corresponding to the endpoint case $p=\infty$ in the noncommutative case. The
associated ${L_p}$ theory is more recent, but it has already produced
important applications. A striking example is the work of Lafforgue and
de la Salle \cite{LD2011},  they proved that the spaces ${L_p}(\mathcal L(SL_3(\mathbb Z)))$ fail to
have the completely bounded approximation property when $p>4$ by using Fourier-Schur multiplier techniques on noncommutative ${L_p}$ spaces. This
provided fundamental examples of noncommutative ${L_p}$ spaces without
CBAP and highlighted the importance of Fourier-Schur multiplier
methods in studying approximation properties of group von Neumann algebras.  Junge, Mei and Parcet \cite{JMP2014} established a H\"ormander-Mihlin theory for  finite-dimensional cocycles with optimal smoothness conditions. Gonz\'alez-P\'erez, Junge and Parcet \cite{GJP2017} established H\"ormander-Mikhlin type \({L_p}\)-multiplier criteria for smooth spectral and non-spectral Fourier multipliers on group algebras of locally compact groups, using noncommutative maximal principles and Sobolev dimension to obtain new \({L_p}\) estimates. Junge, Mei and Parcet \cite{JMP2018} prove that H\"ormander-Mikhlin multipliers on group von Neumann algebras can be represented as Littlewood-Paley averages of noncommutative Riesz transforms, yielding new Sobolev/Besov-type smoothness criteria with dimension-free bounds for arbitrary unimodular groups. Parcet, Ricard and de la Salle \cite{PRD2022} establish precise regularity conditions for \(L_p\)-boundedness of
Fourier multipliers in the group algebra of \(SL_n(\mathbb{R})\) by the H\"ormander-Mikhlin  criterion, and prove a rigidity theorem for radial
multipliers in this setting.
Moreover, for free group von Neumann algebras, the ${L_p}$-theory of Fourier multipliers has also been developed in several directions. In particular, Mei and Ricard \cite{MR2017} studied Hilbert transforms on free groups and proved their complete boundedness on
${L_p}(\mathcal L(\mathbb F_r))$ for  $1<p<\infty$. Later, Mei, Ricard and Xu \cite{MRX2022} established a
Mikhlin multiplier theory for free groups. In particular, their
results show that suitable classical Mikhlin multipliers on $\mathbb Z^d$
give rise to completely bounded Fourier multipliers on
${L_p}(\mathcal L(\mathbb F_\infty))$ for $1<p<\infty$. 



Let \(G=\mathbb F_r\) be the free group generated by \(\{a_1,\cdots,a_r\}\), equipped with the word length function \(|\cdot|\) defined by
\[
 |\gamma | = \inf\left\{n : \gamma = a_{i_1}^{\varepsilon_1} \cdots a_{i_n}^{\varepsilon_n},\ \varepsilon_j \in \{1, -1\}\right\}, \quad \gamma\in \mathbb{F}_r.
\]  Haagerup \cite{Haa1978}  proved  that the reduced \(C^*_r(\mathbb F_r)\) as well as the noncommutative \(L_p(\mathcal L\mathbb F_r)\) admits the completely bounded approximation property (CBAP).  The  existence theorem of Schauder basis of \({L_p}(\mathcal L(\mathbb F_r))\) bases by Junge, Nielsen, Ruan, and Xu  \cite{JNRX2004}.  Whereas the explicit construction of such a basis remains an open problem. The results of Kuhn \cite{K1984} and, independently, of Bo\.zejko and Fendler \cite{BF2006} show that the partial sum operators  
\[S_N(x)=\sum_{|\gamma|\leq N}\hat x(\gamma)\lambda(\gamma),\quad x\in \mathcal L(\mathbb{F}_r)\]
fail to be uniformly bounded on
${L_p}(\mathcal L(\mathbb F_r))$ for $p> 3$ and  $1 \le p < \frac32$, where \(|\gamma|\) is the word length norm  on free groups. However, to the best of our knowledge, whether the family $\{S_N\}_{N\ge 0}$ is uniform bounded on ${L_p}(\mathcal L(\mathbb F_r))$ remains open in the intermediate range 
\(\frac32<p<3\). Further negative evidence was given by Parcet: replacing the standard length with the \(|\gamma|_q=(n_1+\cdots+n_s)^{1/q}\) invalidates such truncation approximations entirely,  where \(\gamma=a_{i_1}^{n_1}\cdots a_{i_s}^{n_s}\), \(i_j\ne i_{j+1}\) and \(q>1\), the case  \(q=1\) is the subject of ongoing work. While related work by Junge, Mei, Ricard, Parcet and collaborators concerns Hilbert and Riesz transforms, this paper focuses on radial multipliers and introduces the free analogue of Rubio de Francia’s mixed norm space.
 For every
$x\in \mathcal L(\mathbb F_r)$, the mixed-norms are defined by
\begin{equation*}
	\begin{aligned}
		\left\|x\right\|_{{L_p}(\mathcal L(\mathbb F_r);
			\mathbb E_{\mathrm{rad}}^c)}
		&:=
		\left\|
		\left(
		\mathbb E_{\mathrm{rad}}
		\big[x^*x\big]
		\right)^{\frac12}
		\right\|_{{L_p}(\mathcal L(\mathbb F_r))},\\
		\left\|x\right\|_{{L_p}(\mathcal L(\mathbb F_r);
			\mathbb E_{\mathrm{rad}}^r)}
		&:=
		\left\|
		\left(
		\mathbb E_{\mathrm{rad}}
		\big[xx^*\big]
		\right)^{\frac12}
		\right\|_{{L_p}(\mathcal L(\mathbb F_r))},
	\end{aligned}
\end{equation*}
where $\mathbb E_{\mathrm{rad}}$ denotes the conditional expectation from
the group von Neumann algebra $\mathcal L(\mathbb F_r)$ onto its radial
subalgebra \textcolor{blue}{$\mathcal L(\mathbb F_r)_{\mathrm{rad}}$}. We refer readers to \cite{JP2010} for more information on mixed-norm spaces. Similarly, using the Iwasawa decomposition \(G=KAN\), Parcet \cite{P2025} introduced a related mixed-norm space \(S_p(AN;E_K)\) and proved that Schur CBAP on this mixed-norm space implies Schur CBAP on \(S_p(G)\), with applications to \(L_p\)-rigidity and Connes \(W^*\)-rigidity of higher-rank lattices.


The following result proves the mixed-norm \(L_p\) boundedness of the partial sum operator \(S_N\) in \(\frac{3}{2} < p < 3 \).

\begin{theorem}\label{Tm-pp}  Let \(r\geq 2\)  and \(\frac{3}{2}< p<3\). Then there exists a universal constant $C_{p,r}>0$ depending only on $p,r$ such that
	\[ \sup_{N\ge0 }\left \| S_N(x) \right \|_{{L_p}(\mathcal{L}(\mathbb{F}_r);\mathbb{E}_{\mathrm{rad}}^c)}\leq C_{p,r} \left \| x \right \|_{{L_p}(\mathcal{L}(\mathbb{F}_r);\mathbb{E}_{\mathrm{rad}}^c)},\]
	for all \(x\in L_p(\mathcal{L}(\mathbb{F}_r);\mathbb{E}_{\mathrm{rad}}^c)\). The analogous assertion also holds for
	\(L_p(\mathcal{L}(\mathbb{F}_r);\mathbb{E}_{\mathrm{rad}}^r)\).
\end{theorem}
A simple duality argument reduces the above problem to deriving elegant noncommutative generalizations of \eqref{T2wM}. This approach is inspired by the weighted  \(L_2\)-estimates in the C\'ordoba and  Feﬀerman framework. Note that \(\mathcal{L}(\mathbb{F}_r)_{\mathrm{rad}} \cong  L^{\infty}(I, dm_r)\) for some explicit measure \(dm_r\) on an interval \(I=[-\frac{\sqrt{2r-1}}{r},\frac{\sqrt{2r-1}}{r}]\).


\begin{theorem}\label{mainthm}
	Let \(r\ge 2\) and \(\alpha>2\).  There exists a constant  \(C_\alpha>0\) only depending on \(\alpha\) such that for every \(x\in \mathcal{L}(\mathbb{F}_r)\) and  \(w\in (\mathcal L(\mathbb F_r)_\mathrm{rad})_+\),  we have
	\begin{equation*} 
		\tau\Big(|S_N(x)|^2\cdot w\Big)\le C_{\alpha}\tau\Big(|x|^2\cdot \mathcal M_\alpha(w)\Big),
	\end{equation*}
	where 
	\[\mathcal M_\alpha(w)=(\Gamma ^{-1}\circ M_\alpha \circ\Gamma )(w)\]
	and 
	\[M_\alpha(G)(s)=\sup_{h>0}\big(\frac{1}{2h}\int_{s-h}^{s+h}|G(t)|^\alpha dt\big)^\frac{1}{\alpha},\quad G \in C(I).\]
\end{theorem}
  Theorem \ref{Tm-pp} can be derived from Theorem \ref{mainthm}, duality arguments, and the \(A_p\)-weighted boundedness of the Hardy–Littlewood maximal operator \(M\). In the Euclidean setting, for any radial function \(g:\mathbb R^n\to\mathbb R\), the weighted \(L_2\) estimates are valid. The maximal operator  in \eqref{T2wM} is the Kakeya maximal function defined by
\[\sup_{\omega\in S^{n-1},h>0}\frac{1}{2h}\int_{-h}^h g(\cdot+t\omega)dt.\]  Theorem \ref{mainthm} reveals the idea of a ``noncommutative" Kakeya maximal function defined on  \(\mathbb F_r\) with respect to the Poisson boundary \((\partial \mathbb{F}_r,\nu)\).
Denote
\[L^2(\mathcal{L}[\mathbb F_r]) = \bigoplus_{m=0}^\infty \bigoplus_{n= m}^\infty V_{m,n}, \]
where \(V_{m,n}\) consists of the \(m\)-th difference components associated with Fourier coefficients supported on the sphere of radius \(n\). \textcolor{blue}{
A function \(\varphi:\mathbb F_r\to\mathbb C\) is called radial if \(\varphi(\gamma)\) depends only on \(|\gamma|\).} For the radial multiplier operator \(T_\varphi\),  the subspaces \(\{V_{m,n}\}_{m\geq0,n\geq m}\) are  invariant  under \(T_\varphi\). Let \(P_{m,n}\) denote the orthogonal projection from
\(L_2(\mathcal L(\mathbb F_r))\) onto \(V_{m,n}\).
Therefore, for every \(x\in \mathcal{L}(\mathbb{F}_r)\), using the decomposition associated with the projections \(P_{m,n}\), we obtain
\[T_\varphi(x)=
		\sum_{m\ge 0}\sum_{n\ge m}
		\varphi(n)
		P_{m,n}(x).\]
In addition, there is a natural filtration on \(\partial \mathbb{F}_r\) defined by  \(\mathcal F_m=\sigma\{E(\gamma ):\gamma \in \mathbb{F}_r\  \mbox{with}\ |\gamma |=m\}.\) Write
\[L_2(\partial \mathbb F_r)= \mathbb{C}\mathds{1} \oplus \bigoplus_{m\ge 1} \bigl(L_2(\mathcal{F}_m) \ominus L_2(\mathcal{F}_{m-1})\bigr) := H_0 \oplus \bigoplus_{m\ge 1} H_m.\]
By Plancherel theory, there exists a representation \(\widetilde{\pi}:\mathbb F_r\to B(L_2(\partial\mathbb F_r))\)  inducing an identification \(\Phi(\lambda(\gamma))(s)=\widetilde{\pi}_{s}(\gamma)\mathds{1}\), where \(\gamma\in\mathbb F_r,s\in I\). Under this map, for each  \(m\ge 0\) and \(n\ge m\), the space \(V_{m,n}\) can be viewed as the tensor product of a one-dimensional function space on the interval \(I\)
and a martingale difference subspace on the Poisson boundary \(\partial \mathbb F_r\). Indeed, there exists a deformed Bo\.zejko–Fendler orthogonal system \(Q_{m,n}\) such that
	\[
\Phi(V_{m,n})=Q_{m,n}\otimes H_m.
\]
Under the isomorphism 
\[\Phi: L_2(\mathcal{L}(\mathbb{F}_r)) \to \bigoplus_{m\ge 0} L_{2}(I, H_m),\]
we have
\[T_\varphi(x)\cong \bigoplus_{m\ge 0}\int_IK_m(\cdot,t)(\Phi(x))_m(t)dm_r(t),\quad x\in L_2(\mathcal L\mathbb F_r),\]
where \(K_m=\sum_{n\ge m}\varphi(n)Q_{m,n}\otimes\bar{Q}_{m,n}:I\times I\to\mathbb C\). Moreover, if \(\varphi=\mathds{1}_{\{n\leq N\}}\), that is, \(T_\varphi=S_N\)  is the partial sum operator, we deduce that the kernel satisfies the decomposition below
\[K_{m,N} \sim \text{weighted kernels of Hilbert transform} + \text{regular parts.}\]
This decomposition is exactly the crucial ingredient enabling the elegant noncommutative generalizations of \eqref{T2wM} presented in Theorem \ref{mainthm}.




==> previous_versions/preliminaries_poisson_bdry_and_reps1.tex <==

\subsection{Poisson boundary and principal series representations}
For the probability measure \(\mu_1\), we define the \(\mu_1\)-Poisson boundary of \(\mathbb{F}_r\) as follows. Let \(\partial \mathbb{F}_r\) be the set of all infinite reduced words in the generators of \(\mathbb{F}_r\). That is, every \(\omega \in \partial \mathbb{F}_r\) is a string \(\omega = a_{i_1}^{\varepsilon_1} a_{i_2}^{\varepsilon_2} \cdots a_{i_n}^{\varepsilon_n} \cdots\) of letters \(a_{i_j} \in \mathbb{F}_r\) with \(|a_{i_j}| = 1\) ,\ \(\varepsilon_{j}= \pm 1\) and \(a_{i_j}^{\varepsilon_j} \neq a_{i_{j+1}}^{-\varepsilon_{j+1}}\) for \(j \ge 1\). 
For \(\gamma  \in \mathbb{F}_r\), denote by \(E(\gamma )\) the set of all \(\omega \in \partial \mathbb{F}_r\) having the first \(|\gamma |\) letters equal to the corresponding letters of the reduced word \(\gamma \). The topology generated by the
cylinder sets
\(
\{E(\gamma ):\gamma \in\mathbb F_r\}
\)
is the natural product topology on \(\partial \mathbb{F}_r\). We denote by
\[
\mathcal F=\sigma\{E(\gamma ):\gamma \in\mathbb F_r\}
\]
the associated Borel \(\sigma\)-algebra.
We define a measure \(\nu\) on the cylinder sets by
\(\nu(E(\gamma ))= 1/c(n)\) with \(|\gamma | = n\). This definition can be extended uniquely to a Borel probability measure on
 \((\partial \mathbb{F}_r,\mathcal F)\) 
The probability space \((\partial \mathbb{F}_r, \mathcal F, \nu)\) is called the Poisson boundary of \(\mathbb{F}_r\).

The finite family of subsets \(\{E(\gamma ):\gamma \in \mathbb{F}_r\  \mbox{with}\  |\gamma |=n\}\) is a partition of \(\partial \mathbb{F}_r\). For each \(n\geq0\), set
\[\mathcal F_n=\sigma\{E(\gamma ):\gamma \in \mathbb{F}_r\  \mbox{with}\ |\gamma |=n\}.\]
Then \((\mathcal F_n)_{n\geq0}\) is a filtration of \(\mathcal F\). For \(\xi\in L^\infty(\partial \mathbb{F}_r,\mathcal F,\nu)\), let \((\mathbb E_n)_{n\geq0}\) denote the conditional expectations  with respect to the filtration \((\mathcal F_n)_{n\geq0}\). They are given by
\[\mathbb E_n(\xi)(\omega)=\sum_{\gamma \in \mathbb{F}_r,|\gamma |=n}\frac{1}{\nu(E(\gamma ))}\int_{E(\gamma )}\xi(\omega)d\nu(\omega)\chi_{E(\gamma )}(\omega),\quad n\geq0,\omega\in\partial \mathbb{F}_r.\]
A sequence \(\xi=(\xi_n)_{n\geq0}\) in \(L^1(\partial \mathbb{F}_r)\) is called a martingale with respect to the filtration \((\mathcal F_n)_{n\geq0}\) if for every \(n\geq0\),
\[\mathbb{E}_n(\xi_{n+1})=\xi_n.\]
For \(n\geq 0\), we define \(\Delta_n(\xi)=\xi_n-\xi_{n-1}\) with convention that \(\xi_{-1}=0\) and \(\mathbb{E}_{-1}=\mathbb{E}_{0}\). The sequence \(\Delta(\xi)=(\Delta_n\xi)_{n\geq0}\) is called the martingale difference.

The free group \(\mathbb{F}_r\) acts naturally on its boundary \(\partial \mathbb{F}_r\), that is \( \Lambda_\gamma (\omega) = \gamma \omega\). And we have \( \Lambda_{\gamma} \circ \Lambda_{\eta } = \Lambda_{ \gamma \eta } \). 
For each \(\gamma  \in \mathbb{F}_r\), we define the measure \(\nu_{\gamma}\) by \(\nu_{\gamma}(E) = \nu(\gamma ^{-1}E)\). 
%Define \(N(\gamma ,\omega)\) as follows:  If \(\omega \in E(\gamma )\), set \(N(\gamma ,\omega) = |\gamma |\).  Otherwise, let \(0 \le N(\gamma ,\omega) = k < |\gamma |\) be the number of initial letters of \(\omega\) that match those of \(\gamma \) before the first mismatch. 
 The Poisson kernel is defined as the Radon--Nikodym derivative
 \[
 P(\gamma,\omega)
 :=
 \frac{d\nu_\gamma}{d\nu}(\omega),
 \quad
 \gamma\in\mathbb F_r,\ \omega\in\partial\mathbb F_r.
 \]
 
The Poisson kernel \(P(\gamma ,\omega)\) satisfies the following properties.
\begin{lemma}{\cite[Chapter 3, Proposition 2.5]{FP1983}}\label{Possion-lem}
Let \(\gamma \in \mathbb{F}_r,\ \omega\in \partial \mathbb{F}_r,\ z\in \mathbb{C}\) and  \( |\gamma | = n \). Then
\begin{align*}
        (P(\gamma , \omega))^z = (2r-1)^{nz} \chi_{E(\gamma^{(n)})}(\omega) & + \sum_{j=1}^{n-1} (2r-1)^{(n-2j)z} \left (\chi_{E(\gamma^{(n-j)})}(\omega)-\chi_{E(\gamma^{(n-j+1)})}
          (\omega)\right)\\&+(2r-1)^{-nz}\left(1- \chi_{E(\gamma^{(1)})}(\omega)\right).
    \end{align*}
\end{lemma}
Let \(J= [0,\pi/\log{(2r-1)}]\). The principle series representations are defined by
\begin{equation}\label{pi-def}
	\pi_z(\gamma )\xi(\omega)\coloneqq \big(P(\gamma ,\omega)\big)^z\xi(\gamma ^{-1}\omega),\quad z\in \frac{1}{2}+\mathrm{i}J,\ \gamma \in \mathbb{F}_r,\ \xi\in L_2(\partial \mathbb{F}_r).
\end{equation}
The function  
\begin{equation}\label{gamma-def}
	F(z) = \frac{1}{2r}\left((2r-1)^z + (2r-1)^{1-z}\right)
\end{equation}
is a bijection from \(\frac{1}{2}+\mathrm{i}J\) to \(I\). Thus we can parameterize the principal representations on \(I\) by defining
\(\widetilde\pi_s\coloneqq\pi_{F^{-1}(s)}\). 
\begin{lemma}{\cite[Page 52]{FP1983}}\label{phi-rep-con}
    The corresponding unitary  representations of the spherical functions \(\{\varphi_s\}_{s\in I}\) are the principal series representations, that is
    \begin{equation*}\label{spericalwithrep}
    	\varphi_s(\gamma)=\langle \widetilde{\pi}_s(\gamma)\mathds{1},\mathds{1}\rangle_{L_2(\partial \mathbb{F}_r)}=\int_{\partial \mathbb{F}_r}P(\gamma,\omega)^{F^{-1}(s)}d\nu(\omega), \quad \gamma\in \mathbb{F}_r,
    \end{equation*}
%    \begin{equation*}\label{spericalwithrep}
%	    L_{\varphi_s}(f)=\sum_{x\in\mathbb F_r}f(x)\langle\widetilde{\pi}_s(x)\mathds{1}, \mathds{1}\rangle_{L^2(\partial \mathbb{F}_r)},\quad
%		f\in \mathbb C[\mathbb{F}_r],
%	\end{equation*}
where \(\mathds{1}(\omega)\equiv 1\) on  \(\partial \mathbb{F}_r\).
\end{lemma}

Define a linear map \(\Phi:\lambda(\mathbb{C}[\mathbb{F}_r])\to L_0(I,dm_r;L_2(\partial \mathbb{F}_r))\) by
	\begin{equation}\label{phi-def}
		\Phi(\lambda(f))(s)= \widetilde{\pi}_s(f)\mathds{1},\quad f\in \mathbb{C}[\mathbb{F}_r],s\in I.
	\end{equation}
	
\begin{lemma}{\cite[Chapter 5, Theorem 4.1]{FP1983}}\label{Plancherelthm}
     The map \(\Phi\) extends to an isometric isomorphism between Hilbert spaces. That is
    \[
    \left\| \Phi(x) \right\|_{L_2(I,dm_r;L_2(\partial \mathbb{F}_r))}=\left\|x\right\|_{L_2(\mathcal{L}(\mathbb{F}_r))},\quad x\in L_2(\mathcal{L}(\mathbb{F}_r)).
    \]
    Moreover, there exists a unitary operator \(U:\ell_2(\mathbb{F}_r) \to L_2(I,dm_r;L_2(\partial \mathbb{F}_r))\) such that
    \[
    \lambda(\gamma ) = U^*\big(\int_{I}^{\oplus} \widetilde{\pi}_{s}(\gamma ) \, dm_r(s)\big) U,\quad \gamma \in \mathbb{F}_r.
    \]
    In particular,
    \begin{equation*}\label{trace-pri-se}
    \tau(\lambda(f))=\int_I L_{\varphi_s}(f)dm_r(s)=\int_I\langle\widetilde{\pi}_s(f)\mathds{1},\mathds{1}\rangle dm_r(s),\quad f\in \mathbb{C} [\mathbb{F}_r].
    \end{equation*}
\end{lemma}

\begin{lemma}\label{Phi}
	For every \(1\leq p<\infty\), the linear map \(\Phi\) extends to an isometric isomorphism between Banach spaces
	\begin{equation*}
		\begin{aligned}
			\Phi :{L_p}(\mathcal{L}(\mathbb{F}_r);\mathbb{E}_{\mathrm{rad}}^c) &\to {L_p}(I,dm_r;L^2(\partial \mathbb{F}_r)).
		\end{aligned}
	\end{equation*}
\end{lemma}
\begin{proof}
	The case \(p=2\) follows immediately from Lemma~\ref{Plancherelthm}. Otherwise, it suffices to prove that \(\Phi\) is an isometry on \( \mathbb{C}[\mathbb{F}_r]\). Let \(f\in \mathbb{C}[\mathbb{F}_r]\). Using Lemma~\ref{phi-mul} (iii),  we obtain
	\[
	\left \| \lambda(f) \right \|_{{L_p}(\mathcal{L}(\mathbb{F}_r);\mathbb{E}_{\mathrm{rad}}^c)}^p = \tau\big( (\mathbb{E}_{\mathrm{rad}}[\lambda(f)^*\lambda(f)])^{\frac{p}{2}}\big) =\int_I L_{\varphi_s}\big((\mathbb{E}_{\mathrm{rad}}[\lambda(f)^*\lambda(f)])^{\frac{p}{2}}\big) dm_r(s).
	\]
	Now Lemma \ref{phi-mul} (i) and  Lemma~\ref{phi-rep-con} yield
	\begin{equation*}
		\begin{aligned}
			\left \| \lambda(f) \right \|_{{L_p}(\mathcal{L}(\mathbb{F}_r);\mathbb{E}_{\mathrm{rad}}^c)}^p & =\int_I \big|L_{\varphi_s}\big(\mathbb{E}_{\mathrm{rad}}[\lambda(f)^*\lambda(f)]\big)\big|^{\frac{p}{2}}  dm_r(s)=\int_I \big|L_{\varphi_s}\big(\lambda(f^**f)\big)\big|^{\frac{p}{2}}  dm_r(s)\\
			&=\int_I \left |\langle \widetilde{\pi}_s(f^**f)\mathds{1},\mathds{1}\rangle_{L^2(\partial \mathbb{F}_r)}\right |^{\frac{p}{2}}dm_r(s) = \int_I\left| \langle \widetilde{\pi}_s(f) \mathds{1}, \widetilde{\pi}_s(f)\mathds{1}\rangle_{L^2(\partial \mathbb{F}_r)} \right|^{\frac{p}{2}}dm_r(s)\\
			& = \int_I \left\| \widetilde{\pi}_s(f) \mathds{1} \right\|_{L^2(\partial \mathbb{F}_r)}^p dm_r(s)  = \left \|\Phi(\lambda(f)) \right\|_{{L_p}(I,dm_r;L^2(\partial \mathbb{F}_r))}.
		\end{aligned}
	\end{equation*}
	Hence, \(\Phi\) is an isometry on \(\mathbb{C}[\mathbb{F}_r]\). Since \(\mathbb{C}[\mathbb{F}_r]\) is dense in \({L_p}(\mathcal{L}(\mathbb{F}_r);\mathbb{E}_{\mathrm{rad}}^c)\), the map \(\Phi\) extends uniquely to an isometric isomorphism from \({L_p}(\mathcal{L}(\mathbb{F}_r);\mathbb{E}_{\mathrm{rad}}^c)\) onto \({L_p}(I,dm_r;L^2(\partial \mathbb{F}_r))\).
\end{proof}






==> previous_versions/preliminaries_radial_algebra1.tex <==

Denote by \(\mathbb{C}[\mathbb{F}_r]\) the family of all the finitely supported complex functions on \(\mathbb{F}_r\). 
For any representation \(\pi\) of \(\mathbb F_r\), we use the same symbol \(\pi\) for its linear extension to finitely supported functions on \(\mathbb F_r\), namely
\[
\pi(f)=\sum_{\gamma\in \mathbb F_r} f(\gamma)\pi(\gamma),
\qquad f\in \mathbb{C}[\mathbb F_r].
\]
%For a fixed $N\in\mathbb{N}$, set $$m_N\coloneqq\chi_{\{x\in\mathbb F_r:\ |x|\leq N\}}.$$ We define the associated Fourier multiplier \(S_N\) by
%\begin{equation*}
%	S_N :\lambda(x) \mapsto \chi_{\{|x|\leq N\}}\lambda(x),\quad x\in  \mathbb{F}_r.    
%\end{equation*}



For each  integer \(n\geq 0\), we let \(c(n)\) denote the number of group elements of length \(n\), that is
\begin{equation}\label{cn-def}
	c(n)\coloneqq \left\{
	\begin{aligned}
		&\ {2r(2r-1)^{n-1}}, & \hbox{ $n\geq1$}, \\
		&\ 1, & \hbox{ $n=0$}.
	\end{aligned}
	\right.
\end{equation}
Let \(\mu_n\) denote the uniform probability measure on the
sphere of radius \(n\), namely
\begin{equation}\label{mu_n}
\mu_{n}\coloneqq \frac{1}{c(n)}\sum_{|\gamma |=n}\delta_{\gamma }.
\end{equation}
The radial sub-algebra \(\mathcal{L}(\mathbb{F}_r)_{\mathrm{rad}}:=\overline{\mathrm{span}\{\lambda(\mu_n):n\ge 0\}}^{w*} \subset \mathcal{L}(\mathbb{F}_r)\) admits a unique trace-preserving conditional expectation given by
\[
\mathbb{E}_{\mathrm{rad}}[x]=\sum_{n=0}^{\infty}\Big(\sum_{|\gamma |=n}\hat x(\gamma)\Big)\lambda(\mu_n),\quad x\in \mathcal L(\mathbb{F}_r).
\]
Throughout the paper, for each \(\gamma\in\mathbb F_r\), we let  \(\gamma^{(n)}\) denote the prefix of \(\gamma\) of length \(n\). For  each \(\gamma \in \mathbb F_r\) with \(|\gamma|=m\) and \(n\ge m\). Set
\begin{equation*}
	s(\gamma ,n)\coloneqq \left\{
	\begin{aligned}
		&\ \{\gamma^{(n)}\}, & \hbox{ $n< m$}, \\
		&\ 	\{\eta \in \mathbb F_r:\ \eta =\gamma \rho,\ |\rho|=n-m,\ |\eta|=n\}, & \hbox{ $n\ge m$}.
	\end{aligned}
	\right.
\end{equation*}
We define projections on \(L_2(\mathcal L(\mathbb F_r))\) as follows. For \(m\ge 0\) and \(x\in \mathcal L(\mathbb{F}_r)\), set
\begin{equation}\label{defEm}
	\mathcal E_m(x)
	\coloneqq
	\sum_{|\eta|<m} \hat{x}(\eta)\lambda(\eta)
	+
	\sum_{n\ge m}\sum_{|\gamma|=m}
	\Big(
	\sum_{\eta\in S(\gamma,n)} \hat{x}(\eta)
	\Big)
	\lambda\left(
	|S(\gamma,n)|^{-1}\chi_{S(\gamma,n)}
	\right).
\end{equation}
Denote
\begin{equation*}
	\mathcal D_m(x)
	\coloneqq
	\mathcal E_m(x)
	-
	\mathcal E_{m-1}(x),
	\quad x\in \mathcal L(\mathbb{F}_r), \ m\ge 0,
\end{equation*}
where we set \(\mathcal E_{-1}=0\). By the above definition, \(\mathcal E_0=\mathbb E_{\mathrm{rad}}\). 


%For each  \(f\in \mathbb{C}[\mathbb{F}_r]\), we define the column and row mixed \(L^p(\ell^2)\)-norms by
%\[
%\left \| \lambda(f) \right \|_{L^p(\mathcal{L}(\mathbb{F}_r);\mathbb{E}_{\mathrm{rad}}^c)} \coloneqq \left \| \big(  \mathbb{E}_{\mathrm{rad}}[\lambda(f)^*\lambda(f)]\big)^{\frac{1}{2}}\right\|_{L^p(\mathcal{L}(\mathbb{F}_r))}
%\]
%and 
%\[
%\left \| \lambda(f) \right \|_{L^p(\mathcal{L}(\mathbb{F}_r);\mathbb{E}_{\mathrm{rad}}^r)} \coloneqq \left \| \big(  \mathbb{E}_{\mathrm{rad}}[\lambda(f)\lambda(f)^*]\big)^{\frac{1}{2}}\right\|_{L^p(\mathcal{L}(\mathbb{F}_r))}.
%\]
%The corresponding mixed \(L^p(\ell^2)\)-spaces are the completions
%of \(\{\lambda(f):f\in\mathbb C[\mathbb F_r]\}\) with respect to these norms.

\begin{lemma}\label{mun}
	Let \(r\geq2\). The sequence \(\{\lambda(\mu_n)\}_{n\geq0}\) satisfies the following recurrence relation
	$$\lambda(\mu_1)\lambda(\mu_n)=\lambda(\mu_n)\lambda(\mu_1)=\frac{1}{2r}\lambda(\mu_{n-1})+\frac{2r-1}{2r}\lambda(\mu_{n+1}), \quad n\ge 1.$$
\end{lemma}
It is known that the spectrum of \(\lambda(\mu_1)\) in \(\mathcal{L}(\mathbb{F}_r)\) is the interval \[I=[-\frac{\sqrt{2r-1}}{r},\frac{\sqrt{2r-1}}{r}].\] 
We denote by
\[
\Gamma : C^*(\lambda(\mu_1)) \longrightarrow C(I)
\]
the Gelfand transform of the commutative \(C^*\)-algebra \(C^*(\lambda(\mu_1))\).
 In view of the preceding lemma, we define a sequence of polynomials on \(I\)
recursively by
\begin{equation}\label{Pn}
	P_0(s)=1,\ P_1(s)=s,\ P_{n+1}(s)=\frac{2r}{2r-1}sP_n(s)-\frac{1}{2r-1}P_{n-1}(s),\quad n\geq1,\ s\in I.
\end{equation}
In fact, the polynomials $\{P_n\}_{n\ge 0}$ coincide with  the Gelfand transform \(\Gamma \) applied to $\{\lambda(\mu_n)\}_{n\ge 0}$. The measure 
\[dm_r(s)=\frac{1}{\pi}\frac{\sqrt{2r-1-r^2s^2}}{1-s^2}ds\]
represents the trace on the radial subalgebra in the sense that for each \(w\in \mathcal{L}(\mathbb{F}_r)_{\mathrm{rad}}\),
\[	\tau(w)=\int_{I}\Gamma (w)(s) dm_r(s).\]
 Moreover, \(\Gamma \) admits an extension to a trace-preserving isomorphism \(\mathcal{L}(\mathbb{F}_r)_{\mathrm{rad}} \cong  L^{\infty}(I, dm_r)\), which is also denoted by \(\Gamma\).
 
 Consider the characteristic equation for the recurrence relation satisfied by the polynomials \(\{P_n(s)\}_{n\ge 0}\), namely
 \[
 X^2-\frac{2r}{2r-1} s X+ \frac{1}{2r-1} = 0.
 \]
 This equation has two roots:
 \begin{equation}\label{sigma-def}
 	\sigma(s)=\frac{rs-\mathrm{i}\sqrt{2r-1-r^2s^2}}{2r-1}\quad \text{and}\quad \bar{\sigma}(s)=\frac{rs+\mathrm{i}\sqrt{2r-1-r^2s^2}}{2r-1}.
 \end{equation}
 Hence, \(\{\sigma(s)^n\}_{n\ge 0}\) and \(\{\bar{\sigma}(s)^n\}_{n\ge 0}\) span the space of functions that satisfy the same recurrence as \(\{P_n(s)\}_{n\ge 0}\). Consequently, for every \(n\ge 0\),
 \begin{equation}\label{Pn-sigma}
 	P_n(s)=\frac{s-{\sigma}(s)}{\bar{\sigma}(s)-\sigma(s)}\,\bar{\sigma}(s)^n+\frac{\bar{\sigma}(s)-s}{\bar{\sigma}(s)-\sigma(s)}\,\sigma(s)^n.
 \end{equation}
 Moreover, due to the orthogonality of \(\{\mu_n\}_{n\ge 0}\), we find that \(\{P_n\}_{n\ge 0}\) forms an orthogonal system in \(L_2(I, dm_r)\).
 
 \begin{lemma}\label{phi-mul} 
 	For each \(s\in I\), define the spherical function 
 	\(\varphi_s :\mathbb F_r\to\mathbb C\) by
 	\[
 	\varphi_s(\gamma )
 	\coloneqq
 	\Gamma \big(\mathbb E_{\mathrm{rad}}(\lambda(\gamma ))\big)(s) = P_{|\gamma|}(s),
 	\qquad \gamma \in\mathbb F_r.
 	\]
 	And define  
 	\[L_{\varphi_s}\big(\lambda(f)\big) =\sum_{\gamma \in\mathbb F_r} f(\gamma )\varphi_s(\gamma ),\] 
 	where \(f\in\mathbb C[\mathbb F_r]\). Then the following assertions hold. 
 	\begin{enumerate}[{\rm (i)}]
 		\item  \(L_{\varphi_s}\) is a character on \(C^*(\lambda(\mu_1))\), and \(L_{\varphi_s}=L_{\varphi_s}\circ\mathbb E_{\mathrm{rad}}\). 
% 		\[
% 		\varphi_s(x)=P_{|x|}(s),
% 		\qquad x\in\mathbb F_r.
% 		\]
% 		
% 		\item For every radial function \(f\in\mathbb C[\mathbb F_r]\),
% 		\[
% 		L_s(\lambda(f))=\Gamma \big(\lambda(f)\big) (s)
% 		=
% 		\sum_{x\in\mathbb F_r} f(x)\varphi_s(x).
% 		\]
 		
 		\item \(\varphi_s\) is a positive definite function on
 		\(\mathbb F_r\) for every \(s\in I\).
 		\item For every \(x\in \mathcal{L}(\mathbb{F}_r)\), 
 		\begin{equation*}
 			\tau(x) =\tau(\mathbb{E}_{\mathrm{rad}}(x))=\int_{I}\Gamma \big(\mathbb E_{\mathrm{rad}}(x)\big)(s)dm_r(s)=\int_{I}L_{\varphi_s}(x) dm_r(s).
 		\end{equation*}
 	\end{enumerate}
 \end{lemma}

% It follows immediately from the definition of \(\varphi_s\) that, for every radial function \(f \in \mathbb{C}[\mathbb{F}_r]\),  the Gelfand transform \(\Gamma \) satisfies
%\[
%\Gamma \big(\lambda(f)\big) (s)= \langle f,\varphi_s\rangle_{\ell^2(\mathbb{F}_r)}.
%\]





